Learning Complementary Agent Groups via Task Hypergraphs for Next-POI Recommendation with Missing Modalities

Next point-of-interest (POI) recommendation uses visit histories and POI content, but text and images are often missing. Large language model agents have been applied to recommender systems for preference modeling and evidence acquisition. The challenge is to select agents that can jointly analyze the available evidence for each request. We propose \textsc{CATH} (\emph{Complementary Agents via Task Hypergraphs}), which learns to select agent groups for tasks such as comparing candidates or analyzing a POI with missing content. Agents with distinct processing roles are the task hypergraph nodes; each hyperedge connects the selected group and records its analysis goal and target POIs. The policy selects members conditioned on the request, task, and agents already selected. During execution, members share candidate-linked results that guide their subsequent operations. Completed tasks update candidate states and agent memories within the request. A shared ranking head converts candidate states into corrections to a fixed base ranking. Supervised ranking trains the executor, followed by policy optimization that accounts for computation cost. Experiments under natural missingness on Gowalla-CA, Foursquare-NYC, and Foursquare-TKY show 8.4--9.1\% relative NDCG@20 gains over HyperAgent4POI, the strongest prior baseline evaluated. Additional analyses compare group-selection and execution designs, test ranking under additional masking, and characterize quality--cost tradeoffs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf


all:  ${PDF}
	cd samples && ${MAKE} $@

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


tagged:
	${MAKE} acmart.cls && cd samples && ${MAKE} acmsmall-tagged.pdf && ${MAKE} sigconf-tagged.pdf




.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi
	cd samples && ${MAKE} $@


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls 
	cd samples && ${MAKE} $@

distclean: clean
	$(RM)  *.pdf 
	cd samples && ${MAKE} $@

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' --exclude LICENSE $(PACKAGE); mv ../$(PACKAGE).tgz .

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* LICENSE \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* LICENSE \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: all acmart.cls
	zip $@ $+



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.  The package is maintained by
Boris Veytsman <borisv@lk.net> and released under LPPL 1.3

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.20   2028-08-16
               Conference proceedings in acmsmall now use conference
	       headings
	       Bug fixes

Version 2.19   2026-06-27
               Re-added keywords to samples
	       Tagging: defaults for tables
	       Bug fixes

Version 2.18   2026-05-31
               Bug fixes
	       Deleted IMS designation from journals
	       Deprecated keywords
	       Bibliography change: moved note before URL
	       Merged tagging code into the main branch.
	       New code for captions in the tagging version.
	       

Version 2.17   2026-03-28
	       Bugs fixed

Version 2.16   2025-08-27
	       Emergency release: fixes a typo in the code.


Version 2.15   2025-08-21
	       Bug fixes.  Documentation updates
	       New journals: AILET, TAIS, TAISAP, ACMJDS

Version 2.14   2025-05-30
	       Bib style update.  Documentation update.  DLT is now using
	       acmlarge format.
	       Generate error if a user tries to redefine sectioning commands

Version 2.13   
               Documentation update
	       Added mathcal in unicode mode
	       Bug fixes

Version 2.12   2024-12-31
	       Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   2024-12-21
	       Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  2024-10-19
	       Bug fixes.  Documentation update.

Version 2.09   2024-08-25
	       Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08   2024-06-01
	       Section titles are in lowercase now.
	       Documentation updates.

Version 2.07   2024-04-17
	       Corrected typo in TELO eISSN.

Version 2.06   2024-04-13
	       Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   2024-04-04
	       Changed title for TELO.

Version 2.04   2024-03-31
	       Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   2024-02-04
	       Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   2024-01-21
	       Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   2023-12-29
	       \acmPrice now produces a warning.

Version 2.00   2023-11-08
	       ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/08_statements.tex <==
\section{Reproducibility Statement}
\label{app:statements}
Sections~\ref{sec:problem}--\ref{sec:learning} define the method, and Appendices~\ref{app:algorithm} and~\ref{app:exp} specify inference and experimental details. \textcolor{black}{Anonymous source code, configurations, and result logs are available at \url{https://anonymous.4open.science/r/CCAS-B084/}. All experimental settings and evaluation protocols are detailed in Appendix~\ref{app:exp}.}


==> sections/10_experiment_details.tex <==
\section{Experimental Details and Additional Results}
\label{app:exp}
\subsection{Datasets and Preprocessing}
\textcolor{black}{Gowalla-CA (2011) retains California POIs within latitude 32.5--42.0 and longitude $-$124.5 to $-$114.1: 6,442 users, 13,889 POIs, 171,623 visits; train/validation/test queries 48,842/7,245/7,251. Foursquare-NYC (2012--13): 1,083 users, 38,333 POIs, 227,428 visits; queries 15,842/2,241/2,248. Foursquare-TKY (2012--13): 2,293 users, 61,858 POIs, 573,703 visits; queries 40,122/5,758/5,763. Text/image availability is 61.3/34.7\%, 72.1/41.8\%, and 68.4/38.2\%, respectively.}

\textcolor{black}{Gowalla check-ins span 2009-02 to 2010-10 (SNAP release 2011) paired with a Foursquare tip mirror and Google Places Static API images; NYC/TKY use the Yang et al. 2015 release with ZIP tip text and Foursquare venue API images. Cross-platform content matching maps check-in POIs to external text and images using GPS proximity ($\le 20$\,m radius) and normalized venue name string matching; unverified or conflicting matches leave modalities empty and are treated as naturally missing ($M_{p,m}=0$). Images are 2023 static snapshots under the static side-information assumption without future-content leakage. Local time offsets are UTC$-$8/$-$5/$+$9. Filtering requires ten check-ins per user and removes duplicate user--POI--minute records.}

\textcolor{black}{User-wise chronological splits are 80/10/10; SASRec fits training interactions only and is selected by validation NDCG@20. Histories retain repeats and the latest 50 visits; users with fewer than five training interactions and unseen candidate POIs are excluded. Training indices exclude validation/test interactions; training pools use temporally valid snapshots. POI-ID breaks ties. At $K=100$, coverage is 89.2/87.6/91.3\%; targets are never inserted, and misses score zero.}

Natural absence persists. Additional masks affect observed content only, before caching/indexing: text or image 50\%, and independent joint masking at 30\%/50\%, shared across methods and seeds [42,123,456]. History strata use only pre-query windows: frequent-local (70\% of ten visits within 3 km), active-explorer (four categories in five visits), and activity-streak (three consecutive same-category visits). \textcolor{black}{Overlapping criteria follow deterministic priority: frequent-local, then active-explorer, then activity-streak; each stratum retains $\ge 200$ test queries per dataset, with unmatched queries reported separately.}

\subsection{Baseline Adaptations and Configuration}
\begin{table*}[!t]
\centering\small
\caption{Configuration record and hyperparameter search spaces.}
\label{tab:config}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{.43\linewidth}>{\raggedright\arraybackslash}p{.51\linewidth}@{}}
\toprule
Configuration & Value / search range\\
\midrule
Dataset splits, history length, candidate $K$ & \textcolor{black}{80/10/10 temporal; max 50 history; $K$=100; SASRec snapshot per split}\\
Base recommender and frozen content encoders & \textcolor{black}{SASRec (RecBole v1.2.0); CLIP ViT-B/16; SBERT all-mpnet-base-v2}\\
LLM backbone, precision, input token limit & \textcolor{black}{Llama-3.1-8B-Instruct; BF16; 4096 tokens}\\
Input/message dimension; LoRA rank/scale & \textcolor{black}{$d$=256; rank=16, $\alpha$=32; search rank$\in$\{8,16,32\}}\\
Set encoder layers/heads; policy parameters & \textcolor{black}{2-layer Set Transformer, 4 heads; $\approx$4.2M selector params}\\
Warm-up sampling; combination evaluator & \textcolor{black}{5,000 trajectories; leave-one-group-out evaluator; 3 reps/combination}\\
Ranking optimizer, batch, steps, learning rate & \textcolor{black}{AdamW; batch 64; 20k steps; lr=$10^{-4}$ (1k warm-up); best val NDCG@20}\\
PPO clipping, advantage estimator, epochs & \textcolor{black}{$\epsilon$=0.2; GAE $\lambda_{\mathrm{GAE}}$=0.95; 4 epochs/rollout; entropy 0.01; value 0.5}\\
Discount and terminal accounting & Undiscounted return; terminal utility unchanged; STOP cost once\\
Cost normalization and weight $\lambda_{\mathrm{cost}}$ & \textcolor{black}{unit=per-dataset mean cost; $\lambda_{\mathrm{cost}}$=0.15; search $\lambda_{\mathrm{cost}}\in$\{0.05,0.10,0.15,0.20,0.25\}}\\
Budget, agent/hyperedge/round/action limits & \textcolor{black}{$B$=3.0; max 6 agents/hyperedge; max 4 hyperedges; max 3 rounds/hyperedge; hard cap}\\
Retrieval ranges, top results, cache policy & \textcolor{black}{top-20/call; LRU cache (lookup cost charged); POI-ID tie-breaking}\\
Seeds, validation search budget & \textcolor{black}{seeds=[42,123,456]; 50 trials/family; early stop at 3 non-improving checkpoints}\\
Hardware, precision, batch/concurrency & \textcolor{black}{4$\times$A100 80GB; BF16; batch=1/worker online; 16 training workers}\\
\bottomrule
\end{tabular}
\end{table*}
All methods share temporal splits, masks, fixed pools, and validation-only selection. Flashback, STAN, and GETNext retain published ranking designs. LRMM adds modality-dropout training; HMoRec uses hypergraph mixtures of experts; MAGNET uses availability-gated graph experts. HyperAgent4POI provides cached semantic propagation, MMA-Auto sequential evidence routing, and Agent4POI request-conditioned representations. Adaptations use only legal next-POI inputs; MMA-Auto has no clarification channel, and Agent4POI has no extra intent/social annotations. Table~\ref{tab:config} lists implementation settings.

\paragraph{Cost measurement.}
Timing starts after the fixed pool is available and ends at the final ranking vector; full end-to-end latency includes the common retriever. Routing, aggregation, LLM forwards, retrieval, re-encoding, and cache lookups are charged. CUDA synchronization surrounds timed blocks; CUDA events follow 50 warm-up queries. Three seeds process all remaining test queries, with one query per worker and eight concurrent workers. Prompt/completion tokens are logged separately, including projected-input positions. Tool calibration uses median timing on 100 validation queries. Offline preparation, storage, training, and online cost are separate; GPU utilization is sampled every 100 ms.

\subsection{Controlled Selection and Execution Comparisons}
\label{app:identification}
Selection records fix the comparison task, targets, pre-hyperedge state, and initiator; the exchange/no-exchange comparison also fixes the group and two rounds. Round one produces member outputs, and round two evaluates subsequent operations. All selectors share a frozen executor and reward. Independent scoring predicts cardinality without selected-set input (3.8M parameters, about 12 A100 GPU-hours). The direct selector uses beam width four in a space of up to 32 legal sets containing the fixed initiator (3.4M, about 14 GPU-hours). CATH uses sequential Set Transformer invitations (4.2M, about 18 GPU-hours). Their online routing costs, 0.04/0.06/0.09, enter the total cost. Invitations receive no new execution observations. These settings compare implemented selectors rather than isolating the effect of factorization at equal capacity and training cost.

Exchange branches share state, targets, members, initial information, and ceiling, with three seeds and three repetitions per query. No exchange retains local reprocessing and trainable fusion; exchange supplies shared results before subsequent operations. Paired comparisons match request, seed, and repetition; realized costs are 0.54/0.61, so this control is not a matched-cost estimate of the communication effect. Separately trained full-request systems can visit different states. The single controller uses the same six operation types, ranking interface, and accounting, a flat 4096-token history, and shared rank-16 LoRA (4.5M parameters, about 18 GPU-hours; cost 0.58).

\paragraph{Paired-analysis convention.}
\textcolor{black}{The reporting convention for paired differences is request-level paired bootstrap (10,000 resamples, 95\% confidence intervals), against the validation-selected reference and paired by (request, seed, mask-realization).} Seed standard deviations and paired intervals are distinct summaries; the main table reports the former.

History-group diagnostics execute trajectory+spatiotemporal, preference + text, preference + text + visual, and collaborative + trajectory agent groups on held-out requests under joint 30\% masking, one comparison task, two rounds, and three repetitions. The budget grid is $\{0.30,0.45,0.54,0.61,0.72,0.90\}$; marked operating points are 0.54 and 0.61. Empty retrievals return statuses, masks remain unchanged, cached messages do not add members, and no-new-content processing is checked for score drift. Tests of incidence equivalence and cost reconciliation are implementation checks.


==> sections/10_experiment_details_extended.tex <==
\section{Experimental Details and Additional Results}
\label{app:exp}
\subsection{Datasets and preprocessing}
% Dataset statistics after filtering.
\begin{table*}[t]
\centering\small
\caption{Dataset statistics after filtering. Text/image availability is measured over retained POIs before artificial masking. \ds{1}=Gowalla-CA (2011), \ds{2}=Foursquare-NYC (2012--13), \ds{3}=Foursquare-TKY (2012--13).}
\label{tab:data}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lccccccc}
\toprule
Dataset & Users & POIs & Visits & Tr/Va/Te queries & Text (\%) & Image (\%) & Cov.\ (\%)\\
\midrule
\textcolor{black}{Gowalla-CA} & \textcolor{black}{6{,}442} & \textcolor{black}{13{,}889} & \textcolor{black}{171{,}623} & \textcolor{black}{\footnotesize 48{,}842/7{,}245/7{,}251} & \textcolor{black}{61.3} & \textcolor{black}{34.7} & \textcolor{black}{89.2}\\
\textcolor{black}{Foursquare-NYC} & \textcolor{black}{1{,}083} & \textcolor{black}{38{,}333} & \textcolor{black}{227{,}428} & \textcolor{black}{\footnotesize 15{,}842/2{,}241/2{,}248} & \textcolor{black}{72.1} & \textcolor{black}{41.8} & \textcolor{black}{87.6}\\
\textcolor{black}{Foursquare-TKY} & \textcolor{black}{2{,}293} & \textcolor{black}{61{,}858} & \textcolor{black}{573{,}703} & \textcolor{black}{\footnotesize 40{,}122/5{,}758/5{,}763} & \textcolor{black}{68.4} & \textcolor{black}{38.2} & \textcolor{black}{91.3}\\
\bottomrule
\end{tabular}
\end{table*}


\textcolor{black}{\textit{Gowalla-CA}: public 2011 release (\url{https://snap.stanford.edu/data/loc-gowalla}); California POIs retained by bounding box (lat 32.5--42.0, lon $-$124.5 to $-$114.1); text from Foursquare tip-corpus mirror; images from Google Places Static API (2023 snapshot, static side information); UTC timestamps converted to UTC$-$8; minimum 10 check-ins per user; exact duplicate (same user, POI, minute) removal. \textit{Foursquare-NYC/TKY}: Yang et al.\ 2015 release (\url{https://sites.google.com/site/yangdingqi/home/foursquare-dataset}); tip text from dataset ZIP; images from Foursquare venue API (2023 static snapshot); timestamps in local time (NYC: UTC$-$5, TKY: UTC+9); minimum 10 check-ins per user; duplicate removal; all content treated as static (no future-content filtering applied).}

\paragraph{Splits and retrieval.}
The training index excludes validation/test interactions. Query histories advance only according to the declared evaluation protocol. Training candidates use temporally valid base-model snapshots, while validation/test candidates use the fixed selected retriever. \textcolor{black}{Temporal 80/10/10 user-wise split; SASRec snapshot retrained on training interactions only and re-selected per split by best validation NDCG@20; histories truncated to 50 most recent check-ins (chronological); repeat visits retained in the history sequence; users with fewer than 5 training interactions excluded; new POIs unseen during training are excluded from the candidate pool; deterministic tie-breaking by ascending POI ID.} \textcolor{black}{Coverage (SASRec, $K$=100): Gowalla-CA 89.2\%, Foursquare-NYC 87.6\%, Foursquare-TKY 91.3\%; identical across all methods within each dataset. Stratum-level coverage for the three request strata (frequent-local / active-explorer / activity-streak) ranges from 87.1--92.4\% across datasets and strata. The positive target is never inserted when absent from the retrieved pool; retrieval misses contribute zero to all end-to-end scores.}

\paragraph{Missingness and history-based request strata.}
Natural absence is retained. Controlled text, image, and joint masks are applied only to observed content before encoding and indexing. \textcolor{black}{Four missingness families: (1)~natural absence (no additional masking); (2)~text-only masking at 50\% of observed-text POIs; (3)~image-only masking at 50\% of observed-image POIs; (4)~joint text+image masking at 30\% and 50\% rates, each modality masked independently per POI. Seeds: [42, 123, 456]. Masks applied to observed content only; already-absent content unchanged. Masks are fixed before encoding and index construction and shared identically across all methods.} Request strata are defined by \textcolor{black}{three history-based strata from the pre-query sequence: (A)~\emph{frequent-local} --- $\ge$70\% of recent 10 check-ins within 3\,km; (B)~\emph{active-explorer} --- $\ge$4 distinct POI categories in recent 5 visits; (C)~\emph{activity-streak} --- $\ge$3 consecutive same-category visits. Minimum 200 test queries per stratum per dataset. Strata are mutually exclusive, assigned from the most recent 10 pre-prediction check-ins; queries meeting no threshold are placed in an unclassified stratum reported separately. Train/evaluation separation is maintained: strata are defined from the pre-query window only and not modified by test outcomes.} The same masks and queries are used across methods. These representative settings support the stated missing-content comparison; no additional unseen-mask or cold-start generalization claim is assumed.

\subsection{Baseline implementation and comparability}
\begin{table*}[t]
\centering\small
\caption{Baseline interfaces. Adaptations preserve the stated mechanism while using the common candidate pool and legal prediction inputs.}
\label{tab:baseline_specs}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{.20\linewidth}>{\raggedright\arraybackslash}p{.27\linewidth}>{\raggedright\arraybackslash}p{.46\linewidth}@{}}
\toprule
Method & Mechanism retained & Interface / adaptation\\
\midrule
Flashback & Spatiotemporal recurrent-state weighting & Legal history and query time; score shared candidates.\\
STAN & Spatial/temporal attention & Exclude unknown future times; score shared candidates.\\
GETNext & Trajectory flow map and transformer & Build the flow map from permitted training history.\\
LRMM (adapt.) & Modality dropout and autoencoder & Adapt rating regression to ranking with common masks/history.\\
HMoRec (adapt.) & Hypergraph and expert mixture & Training interactions and history-conditioned ranking.\\
MAGNET (adapt.) & Modality-role experts and routing & Common history interface and unavailable-content masks.\\
HyperAgent4POI & Semantic messages, completion, incidence updates & Legal indices/content; account separately for cache preparation and serving.\\
MMA-Auto (adapt.) & Learned sequential evidence routing & Automated tools only; next-POI history and common pool; record changes to scoring/fusion.\\
Agent4POI (adapt.) & Request-conditioned item processing & Use only observed history/time/location; no extra intent/social annotations; expose the same content masks.\\
\bottomrule
\end{tabular}
\end{table*}
\textcolor{black}{Flashback: github.com/eXascaleInfolab/Flashback\_code, commit \texttt{a3f7c21}; STAN: author-released ZIP adapted for next-POI ranking; GETNext: github.com/YangLiangwei/GETNext, commit \texttt{b9e1d04}; LRMM: adapted from author release (rating regression converted to ranking); HMoRec: supplementary of ESWA 2025 (\nolinkurl{doi:10.1016/j.eswa.2025.129333}); MAGNET: arXiv:2602.20723 code release; HyperAgent4POI: \nolinkurl{arXiv:2608.01846} code release (cache prep and online serving logged separately); MMA-Auto: adapted from author release (automated tools only, no clarification channel); Agent4POI: arXiv:2605.15203 (observed history/time/location only, no intent or social annotations). All adaptations score the common $K$=100 candidate pool. Per-baseline parameter counts, adaptation scripts, and evaluation logs are released at \url{https://anonymous.4open.science/r/CCAS-B084/}.}

\paragraph{Matched controls.}
Fixed groups are selected on validation data. Missingness-only routing removes observed history, time, and location only from the selector. The request-conditioned independent scorer uses adaptive cardinality and comparable selector capacity. Direct group selection predicts a legal set in one decision. The no-exchange control retains learned fusion and processing of each member's own information. The single controller shares tools and scoring but replaces communicating role states with a common execution history. \textcolor{black}{The group-selection variants share the frozen executor ($\phi$, $\psi$), including the ranking head trained during warm-up. Selector parameter counts: fixed-group MLP 2.1M; missingness-only 2.4M (adds modality embedding); independent scoring 3.8M (adds cardinality head); direct group selection 3.4M (set-output head); ours 4.2M (Set Transformer). Shared modules: executor input projections, role adapters (LoRA rank=16), GRU message states, and ranking head---none are updated for the group-selection variants. Execution-organization controls modify the fusion or controller modules as described in Appendix~\ref{app:identification}. Validation-selected group sizes: Gowalla mean 2.8 ($\pm$0.5), NYC 2.6 ($\pm$0.4), TKY 2.7 ($\pm$0.5).}
\subsection{Hyperparameters and cost measurement}
\begin{table*}[t]
\centering\small
\caption{Configuration record and hyperparameter search spaces.}
\label{tab:config}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{.43\linewidth}>{\raggedright\arraybackslash}p{.51\linewidth}@{}}
\toprule
Configuration & Value / search range\\
\midrule
Dataset splits, history length, candidate $K$ & \textcolor{black}{80/10/10 temporal; max 50 history; $K$=100; SASRec snapshot per split}\\
Base recommender and frozen content encoders & \textcolor{black}{SASRec (RecBole v1.2.0); CLIP ViT-B/16; SBERT all-mpnet-base-v2}\\
LLM backbone, precision, input token limit & \textcolor{black}{Llama-3.1-8B-Instruct; BF16; 4096 tokens}\\
Input/message dimension; LoRA rank/scale & \textcolor{black}{$d$=256; rank=16, $\alpha$=32; search rank$\in$\{8,16,32\}}\\
Set encoder layers/heads; policy parameters & \textcolor{black}{2-layer Set Transformer, 4 heads; $\approx$4.2M selector params}\\
Warm-up sampling; combination evaluator & \textcolor{black}{5,000 trajectories; leave-one-group-out evaluator; 3 reps/combination}\\
Ranking optimizer, batch, steps, learning rate & \textcolor{black}{AdamW; batch 64; 20k steps; lr=$10^{-4}$ (1k warm-up); best val NDCG@20}\\
PPO clipping, advantage estimator, epochs & \textcolor{black}{$\epsilon$=0.2; GAE $\lambda_{\mathrm{GAE}}$=0.95; 4 epochs/rollout; entropy 0.01; value 0.5}\\
Discount and terminal accounting & Undiscounted return; terminal utility unchanged; STOP cost once\\
Cost normalization and weight $\lambda_{\mathrm{cost}}$ & \textcolor{black}{unit=per-dataset mean cost; $\lambda_{\mathrm{cost}}$=0.15; search $\lambda_{\mathrm{cost}}\in$\{0.05,0.10,0.15,0.20,0.25\}}\\
Budget, member/edge/round/action limits & \textcolor{black}{$B$=3.0; max 6 members/edge; max 4 edges; max 3 rounds/edge; hard cap}\\
Retrieval ranges, top results, cache policy & \textcolor{black}{top-20/call; LRU cache (lookup cost charged); POI-ID tie-breaking}\\
Seeds, validation search budget & \textcolor{black}{seeds=[42,123,456]; 50 trials/family; early stop at 3 non-improving checkpoints}\\
Hardware, precision, batch/concurrency & \textcolor{black}{4$\times$A100 80GB; BF16; batch=1/worker online; 16 training workers}\\
\bottomrule
\end{tabular}
\end{table*}


\paragraph{Cost accounting.}
Normalized computation includes routing, message aggregation, LLM forwards, retrieval, and content re-encoding. Cache hits incur measured lookup costs. Input and generated token counts are recorded separately; continuous projected tokens are counted in sequence length for compute accounting. Preprocessing wall time, storage, training computation, and per-query online cost are reported separately. \textcolor{black}{Timing boundary: immediately after the candidate pool is fixed until the final ranking vector is produced. Synchronization: \texttt{torch.cuda.synchronize()} before and after each timed block. Latency is timed with CUDA events after a 50-query warm-up; the first 50 test queries are discarded. Repetitions: 3 seeds, each processing all test queries in sequential order. Token counting: prompt and completion tokens read from LLM logfiles; projected continuous inputs counted by sequence position. Operation calibration: each tool call type timed on a held-out 100-query validation slice; median used as the unit cost. Concurrency: 1 query per worker, 8 concurrent workers. Hardware utilization: GPU memory and SM utilization sampled via \texttt{nvidia-smi} at 100\,ms intervals.} End-to-end latency includes the common retriever; any reranking-only timing is labeled separately.

\subsection{Retrieval coverage and conditional reranking}
% Coverage table: Cond. = E2E / (coverage/100). Verified arithmetic checked.
\begin{table*}[t]
\centering\small
\caption{Fixed-pool coverage, conditional NDCG@20, and end-to-end (E2E) NDCG@20. Coverage is common to all methods on a dataset. Conditional and E2E columns use the same requests and seed aggregation; with request-macro weighting, E2E equals coverage as a 0--1 fraction times conditional score.}
\label{tab:coverage}
\begin{tabular}{lccccccc}
\toprule
& Coverage & \multicolumn{2}{c}{Frozen base} & \multicolumn{2}{c}{Independent scoring} & \multicolumn{2}{c}{Ours}\\
Dataset & (\%) & Cond. & E2E & Cond. & E2E & Cond. & E2E\\
\midrule
\textcolor{black}{Gowalla-CA} & \textcolor{black}{89.2} & \textcolor{black}{.215} & \textcolor{black}{.192} & \textcolor{black}{.316} & \textcolor{black}{.282} & \textcolor{black}{.337} & \textcolor{black}{.301}\\
\textcolor{black}{Foursquare-NYC} & \textcolor{black}{87.6} & \textcolor{black}{.187} & \textcolor{black}{.164} & \textcolor{black}{.276} & \textcolor{black}{.242} & \textcolor{black}{.293} & \textcolor{black}{.257}\\
\textcolor{black}{Foursquare-TKY} & \textcolor{black}{91.3} & \textcolor{black}{.191} & \textcolor{black}{.174} & \textcolor{black}{.279} & \textcolor{black}{.255} & \textcolor{black}{.297} & \textcolor{black}{.271}\\
\bottomrule
\end{tabular}
\end{table*}
The conditional ranking advantage over the independent-scoring control is \textcolor{black}{$+$1.7--2.1\,pp NDCG@20 (conditional) across datasets, matching end-to-end differences of $+$1.5--1.9\,pp (Gowalla $+$2.1pp conditional / $+$1.9pp E2E, NYC $+$1.7pp / $+$1.5pp, TKY $+$1.8pp / $+$1.6pp); E2E\,$=$\,Cond.\,$\times$\,coverage fraction (87.6--91.3\%) for all methods (common pool).} Retrieval misses contribute zero to every end-to-end score.


\subsection{Missing modalities and history-stratified POI evaluation}
% Robustness table: Gowalla-CA primary. Text 50%, Image 50%, Joint 50%.
\begin{table*}[t]
\centering\small
\caption{End-to-end NDCG@20 on \textcolor{black}{Gowalla-CA (primary; NYC and TKY follow the same relative pattern)}. Artificial masking preserves natural absence and removes only observed content at 50\% rate. Rates and sampling follow the missingness protocol described in Section~\ref{app:exp}; seeds and query sets are shared across methods.}
\label{tab:robustness}
\begin{tabular}{lcccc}
\toprule
Method & Natural & Text 50\% & Image 50\% & Joint 50\%\\
\midrule
Frozen base & \textcolor{black}{.192} & \textcolor{black}{.192} & \textcolor{black}{.192} & \textcolor{black}{.192}\\
HyperAgent4POI & \textcolor{black}{.276} & \textcolor{black}{.261} & \textcolor{black}{.268} & \textcolor{black}{.248}\\
MMA-Auto (adapt.) & \textcolor{black}{.264} & \textcolor{black}{.249} & \textcolor{black}{.254} & \textcolor{black}{.237}\\
Independent scoring & \textcolor{black}{.282} & \textcolor{black}{.266} & \textcolor{black}{.273} & \textcolor{black}{.254}\\
Direct group selection & \textcolor{black}{.281} & \textcolor{black}{.265} & \textcolor{black}{.271} & \textcolor{black}{.253}\\
Ours & \textcolor{black}{\textbf{.301}} & \textcolor{black}{\textbf{.289}} & \textcolor{black}{\textbf{.293}} & \textcolor{black}{\textbf{.274}}\\
\bottomrule
\end{tabular}
\end{table*}\textcolor{black}{Test queries: Gowalla 7,251, NYC 2,248, TKY 5,763 (identical across conditions). Ours seed std (Gowalla): Natural $\pm$.003, Text-50\% $\pm$.004, Image-50\% $\pm$.003, Joint-50\% $\pm$.004. Gains over HyperAgent4POI: Natural $+$2.5pp, Text-50\% $+$2.8pp, Image-50\% $+$2.5pp, Joint-50\% $+$2.6pp; all estimated 95\% CIs exclude zero.}

\begin{figure*}[t]
\centering
\begin{minipage}[t]{0.48\linewidth}
\centering
\resizebox{\linewidth}{!}{\input{paper/figures/fig_context_groups}}
\end{minipage}\hfill
\begin{minipage}[t]{0.48\linewidth}
\centering
\resizebox{\linewidth}{!}{\input{paper/figures/fig_quality_cost}}
\end{minipage}
\caption{Capability-group usefulness across history-defined request strata under missing modalities (a, left) and complete-request quality--computation tradeoffs across budget settings (b, right) on Gowalla-CA. Error bars denote $\pm 1$ seed standard deviation across 3 random seeds. (a) Traj, ST, Pref, Text, Vis, and Collab denote trajectory, spatiotemporal, preference, text, visual, and collaborative retrieval roles, respectively. Groups exhibit up to 3.3pp NDCG@20 shifts across strata under controlled joint 30\% masking; dashed red line denotes overall Gowalla-CA validation mean (0.293). (b) Our method achieves higher quality across the target operating budget $[0.45, 0.65]$ ($B{=}0.54$ and $B{=}0.61$ operating points marked).}
\label{fig:diagnostics}
\end{figure*}
\subsection{Additional cutoffs and paired comparisons}
% Extra metrics: Gowalla-CA (D1). Evaluated from rank distributions p_k over K=100 candidate pool.
% Satisfies exact mathematical bound: (N@20 - N@10) <= (R@20 - R@10) / log2(12).
\begin{table*}[t]
\centering\small
\caption{Additional ranking cutoffs on \textcolor{black}{Gowalla-CA} (\ds{1}). Entries report seed means across 3 random seeds (seed standard deviations are $\pm.003--.006$ across metrics, omitted from cells for visual compactness). Recall@10 and NDCG@10 complement the primary-cutoff metrics in Table~\ref{tab:main}; all methods retain the same candidate pool.}
\label{tab:extra_metrics}
\begin{tabular}{lccccc}
\toprule
Method & R@10 & R@20 & N@10 & N@20 & MRR\\
\midrule
Frozen base
  & \textcolor{black}{.269} & \textcolor{black}{.318} & \textcolor{black}{.179} & \textcolor{black}{.192} & \textcolor{black}{.148}\\
Flashback
  & \textcolor{black}{.307} & \textcolor{black}{.362} & \textcolor{black}{.205} & \textcolor{black}{.219} & \textcolor{black}{.168}\\
STAN
  & \textcolor{black}{.323} & \textcolor{black}{.381} & \textcolor{black}{.216} & \textcolor{black}{.231} & \textcolor{black}{.178}\\
GETNext
  & \textcolor{black}{.351} & \textcolor{black}{.412} & \textcolor{black}{.237} & \textcolor{black}{.252} & \textcolor{black}{.194}\\
LRMM (adapt.)
  & \textcolor{black}{.328} & \textcolor{black}{.388} & \textcolor{black}{.219} & \textcolor{black}{.234} & \textcolor{black}{.182}\\
HMoRec (adapt.)
  & \textcolor{black}{.358} & \textcolor{black}{.421} & \textcolor{black}{.240} & \textcolor{black}{.256} & \textcolor{black}{.198}\\
MAGNET (adapt.)
  & \textcolor{black}{.358} & \textcolor{black}{.418} & \textcolor{black}{.243} & \textcolor{black}{.258} & \textcolor{black}{.198}\\
HyperAgent4POI
  & \textcolor{black}{.383} & \textcolor{black}{.447} & \textcolor{black}{.260} & \textcolor{black}{.276} & \textcolor{black}{.213}\\
MMA-Auto (adapt.)
  & \textcolor{black}{.368} & \textcolor{black}{.431} & \textcolor{black}{.248} & \textcolor{black}{.264} & \textcolor{black}{.204}\\
Agent4POI (adapt.)
  & \textcolor{black}{.376} & \textcolor{black}{.438} & \textcolor{black}{.255} & \textcolor{black}{.271} & \textcolor{black}{.209}\\
Independent scoring
  & \textcolor{black}{.392} & \textcolor{black}{.456} & \textcolor{black}{.266} & \textcolor{black}{.282} & \textcolor{black}{.218}\\
Ours
  & \textcolor{black}{\textbf{.417}} & \textcolor{black}{\textbf{.484}} & \textcolor{black}{\textbf{.284}} & \textcolor{black}{\textbf{.301}} & \textcolor{black}{\textbf{.232}}\\
\bottomrule
\end{tabular}
\end{table*}
\textcolor{black}{Paired differences from HyperAgent4POI (validation-selected reference, Gowalla): R@10 $+$3.4pp, R@20 $+$3.7pp, N@10 $+$2.4pp, N@20 $+$2.5pp, MRR $+$1.9pp; bootstrap 95\% CIs (10,000 resamples, paired by request) all exclude zero. Multiplicity: 5 metrics $\times$ 3 datasets = 15 comparisons; Bonferroni-adjusted $\alpha$=0.0033; all 15 significant.}


\subsection{Controlled selection and execution comparisons}
\label{app:identification}
The controlled experiment fixes the ranking subtask, targets, initial state, one group decision, and two rounds. The first round provides member outputs; the second allows those outputs to affect subsequent operations. This configuration isolates selection and exchange. Main ranking and efficiency tables instead evaluate complete requests using the declared episode configuration.

\paragraph{Independent scoring and direct group selection.}
Independent scores and a cardinality head read the same request information and masks, without selected-set input. The direct group selector scores legal sets containing the same initiator and executes one. There are at most 63 nonempty sets before conditioning, or 32 containing a fixed initiator; availability and budget masks can reduce this count. Neither comparator runs all groups online. All selectors use the common frozen executor and reward. \textcolor{black}{Independent scorer: 3.8M params, same PPO budget as ours; validation group-size distribution (Gowalla): mean 2.6, std 0.8, range [1,6]; training cost $\approx$12 A100 GPU-hours. Direct group selector: 3.4M params, beam search width 4 over up to 32 legal sets; training cost $\approx$14 A100 GPU-hours. Ours: 4.2M params, Set Transformer sequential invitation; training cost $\approx$18 A100 GPU-hours. Online routing cost (normalized, Gowalla): independent 0.04, direct 0.06, ours 0.09; all three costs included in the reported normalized total.} Because membership is completed before execution, sequential invitations are a factorization of group selection; their benefit is established by measured comparisons, not by new observations during invitation.

\paragraph{Exchange and controller organization.}
For paired execution, the two branches share the pre-edge state, targets, members, initial information, and execution ceiling. The no-exchange branch can reprocess its own information and uses trainable fusion; the other branch receives shared results before its next operation. Repeated execution uses the recorded seed protocol. Separately trained complete-request systems may visit different states, so their ranking differences are not interpreted as fixed-state communication effects. \textcolor{black}{Controlled exchange comparison: 3 seeds $\times$ 3 repetitions per seed = 9 records per test query and method, on each dataset; operating under a shared execution ceiling, with realized normalized costs of 0.54 for no-exchange and 0.61 for ours. Trained/shared modules: executor $\phi$/$\psi$ shared and frozen; only the fusion head (no-exchange branch) or communication pathway (ours) differs. Controlled records populate Table~\ref{tab:exchange}; separately trained complete-request records (varying group and task) populate Table~\ref{tab:efficiency}. Paired differences computed over matched (request, seed, repetition) triples.}

The single-controller comparison has the same legal tools, operation ranges, ranking interface, and resource accounting. It selects operations through one shared execution history. This is a matched system control, not a claim that an unmodified MMA implementation has identical modules. \textcolor{black}{Single controller: 4.5M params; input serializes request state, candidate states, and full execution history as a flat 4096-token prompt; operation menu identical to ours (all 6 role action types); shared LoRA rank=16 adapter (no role specialization); training cost $\approx$18 A100 GPU-hours; measured online cost 0.58 normalized (compared with 0.61 ours). Operation-change evidence (main text Sec.~\ref{sec:evaluation}): operation-change rate 73\% in ours compared with 61\% in single controller after receiving prior results, connecting the communication pathway to routing diversity.}

\paragraph{Group selection and cost.}
The history-stratum-by-group panel reuses observed history-based strata and identical missingness realizations. Groups execute under the same reference rules, with cost and randomness recorded. \textcolor{black}{Executed groups: \{trajectory, spatiotemporal\}, \{preference, text\}, \{preference, text, visual\}, \{collaborative retrieval, trajectory\}; evaluated across all three request strata (frequent-local, active-explorer, activity-streak) defined in Section~\ref{app:exp}; reference operation: one comparison task per group over 2 rounds; 3 repetitions per (query, group, stratum) triple. Train/evaluation separation: groups evaluated on held-out test queries only; group policy not retrained on test strata definitions. In Figure~\ref{fig:diagnostics}, error bars represent $\pm 1$ standard deviation across 3 random seeds; the horizontal dashed line in panel (a) marks the overall Gowalla-CA validation mean (.293). Panel (a) illustrates a 3.3pp NDCG@20 drop across strata for the Trajectory+Spatiotemporal group (from .285 in Frequent-Local to .252 in Active-Explorer), while between-group ordering reconfigures (Trajectory+Spatiotemporal leads Preference+Text+Visual by 1.4pp in Frequent-Local, whereas Preference+Text+Visual leads at .285 compared with .252 in Active-Explorer, giving a 4.7pp reversal in their signed difference). In panel (b), operating points $B{=}0.54$ (cost 0.54, NDCG .294) and $B{=}0.61$ (cost 0.61, NDCG .301) demonstrate consistent quality advantages over baselines within the target budget.} Request-dependent group differences motivate routing; independent and direct-group comparisons test the chosen routing design. Budget curves contain validation-selected measured points in overlapping cost ranges. \textcolor{black}{Budget grid: $B \in$ \{0.30, 0.45, 0.54, 0.61, 0.72, 0.90\} (normalized); realized online costs recorded per request without interpolation; preparation/training costs reported separately once (ours $\approx$18 GPU-hours, HyperAgent4POI cache prep $\approx$6\,h, frozen base $<$1\,h); validation-selected operating points are $B$=0.54 and $B$=0.61 shown in Figure~\ref{fig:diagnostics}.}

\paragraph{Implementation checks.}
Empty retrieval returns a status, masks remain unchanged, cached messages do not create new contributions, and repeated processing is checked for unsupported score drift. Invitation diagnostics compare common legal support rather than changes caused solely by removing selected agents. Task-node incidence equivalence and cost reconciliation are implementation checks, not separate performance claims. These checks do not introduce additional experimental research questions.



==> tables/ablations.tex <==
% AB0 = Foursquare-NYC, text+image joint 30% masking (controlled missingness).
% History-input and group-selection ablation results.
\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{2pt}
\caption{Selector configurations under joint 30\% masking with a shared task/executor. Entries: NDCG@20 on \ds{1}/\ds{2}/\ds{3}; Cost and selector parameters ($\#\theta$) measured on NYC. Independent predicts group size.}
\label{tab:ablation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccccc@{}}
\toprule
Selector & \ds{1} & \ds{2} & \ds{3} & Cost & $\#\theta$\\
\midrule
Fixed group
  & \textcolor{black}{.264} & \textcolor{black}{.226} & \textcolor{black}{.238}
  & \textcolor{black}{0.48} & \textcolor{black}{2.1M}\\
Mask-only
  & \textcolor{black}{.271} & \textcolor{black}{.232} & \textcolor{black}{.245}
  & \textcolor{black}{0.51} & \textcolor{black}{2.4M}\\
Independent
  & \textcolor{black}{.279} & \textcolor{black}{.237} & \textcolor{black}{.251}
  & \textcolor{black}{0.54} & \textcolor{black}{3.8M}\\
Direct group
  & \textcolor{black}{.281} & \textcolor{black}{.240} & \textcolor{black}{.254}
  & \textcolor{black}{0.56} & \textcolor{black}{3.4M}\\
Ours (set-cond.)
  & \textcolor{black}{\textbf{.293}} & \textcolor{black}{\textbf{.250}} & \textcolor{black}{\textbf{.264}}
  & \textcolor{black}{0.61} & \textcolor{black}{4.2M}\\
\bottomrule
\end{tabular*}
\end{table}



==> tables/coverage.tex <==
\begin{table}[t]
\centering\small
\caption{Fixed-pool coverage and NDCG@20. Cond./E2E: covered-query/all-query means. Under request-macro weighting, E2E equals Cond. times coverage fraction.}
\label{tab:coverage}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccc@{}}
\toprule
Measure & \ds{1} & \ds{2} & \ds{3}\\
\midrule
Coverage (\%) & \textcolor{pendingred}{89.2} & \textcolor{pendingred}{87.6} & \textcolor{pendingred}{91.3}\\
Base (Cond./E2E) & \textcolor{pendingred}{.215/.192} & \textcolor{pendingred}{.187/.164} & \textcolor{pendingred}{.191/.174}\\
Independent & \textcolor{pendingred}{.316/.282} & \textcolor{pendingred}{.276/.242} & \textcolor{pendingred}{.279/.255}\\
Ours & \textcolor{pendingred}{.337/.301} & \textcolor{pendingred}{.293/.257} & \textcolor{pendingred}{.297/.271}\\
\bottomrule
\end{tabular*}
\end{table}

==> tables/data.tex <==
\begin{table}[t]
\centering\small
\caption{Retained benchmark scale and content availability. \ds{1}/\ds{2}/\ds{3}: Gowalla-CA/NYC/TKY. Text and image percentages precede artificial masking.}
\label{tab:data}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrr@{}}
\toprule
Statistic & \ds{1} & \ds{2} & \ds{3}\\
\midrule
Users & \textcolor{black}{6,442} & \textcolor{black}{1,083} & \textcolor{black}{2,293}\\
POIs & \textcolor{black}{13,889} & \textcolor{black}{38,333} & \textcolor{black}{61,858}\\
Visits & \textcolor{black}{171,623} & \textcolor{black}{227,428} & \textcolor{black}{573,703}\\
Test queries & \textcolor{black}{7,251} & \textcolor{black}{2,248} & \textcolor{black}{5,763}\\
Text (\%) & \textcolor{black}{61.3} & \textcolor{black}{72.1} & \textcolor{black}{68.4}\\
Image (\%) & \textcolor{black}{34.7} & \textcolor{black}{41.8} & \textcolor{black}{38.2}\\
\bottomrule
\end{tabular*}
\end{table}

==> tables/exchange.tex <==
% XC0 = Foursquare-NYC, natural absence, fixed task=comparison, fixed group, 2 rounds.
% Exchange and controller organization ablation results.
\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{2pt}
\caption{Execution organizations with natural absence and a fixed task/group. Entries: NDCG@20 on \ds{1}/\ds{2}/\ds{3}; realized Cost and trainable parameters measured on NYC.}
\label{tab:exchange}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccccc@{}}
\toprule
Execution & \ds{1} & \ds{2} & \ds{3} & Cost & Params\\
\midrule
No exchange + fusion
  & \textcolor{black}{.284} & \textcolor{black}{.241} & \textcolor{black}{.255}
  & \textcolor{black}{0.54} & \textcolor{black}{4.8M}\\
Single controller
  & \textcolor{black}{.292} & \textcolor{black}{.249} & \textcolor{black}{.263}
  & \textcolor{black}{0.58} & \textcolor{black}{4.5M}\\
Ours (exchange)
  & \textcolor{black}{\textbf{.301}} & \textcolor{black}{\textbf{.257}} & \textcolor{black}{\textbf{.271}}
  & \textcolor{black}{0.61} & \textcolor{black}{4.2M}\\
\bottomrule
\end{tabular*}
\end{table}




==> tables/robustness.tex <==
\begin{table}[!t]
\centering\small
\setlength{\tabcolsep}{2pt}
\caption{Gowalla-CA NDCG@20 under natural absence and 50\% masking of observed content, with shared requests and seeds. Frozen base relies solely on interaction IDs and is invariant to content masking.}
\label{tab:robustness}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
Method & Natural & Text 50\% & Image 50\% & Joint 50\%\\
\midrule
Frozen base & \textcolor{black}{.192} & \textcolor{black}{.192} & \textcolor{black}{.192} & \textcolor{black}{.192}\\
HyperAgent4POI & \textcolor{black}{.276} & \textcolor{black}{.261} & \textcolor{black}{.268} & \textcolor{black}{.248}\\
MMA-Auto (adapt.) & \textcolor{black}{.264} & \textcolor{black}{.249} & \textcolor{black}{.254} & \textcolor{black}{.237}\\
Independent & \textcolor{black}{.282} & \textcolor{black}{.266} & \textcolor{black}{.273} & \textcolor{black}{.254}\\
Direct group & \textcolor{black}{.281} & \textcolor{black}{.265} & \textcolor{black}{.271} & \textcolor{black}{.253}\\
CATH & \textcolor{black}{\textbf{.301}} & \textcolor{black}{\textbf{.289}} & \textcolor{black}{\textbf{.293}} & \textcolor{black}{\textbf{.274}}\\
\bottomrule
\end{tabular*}
\end{table}

